Rank Reduction in Bimatrix Games

The rank of a bimatrix game is defined as the rank of the sum of the payoff matrices of the two players. The rank of a game is known to impact both the most suitable computation methods for determining a solution and the expressive power of the game. Under certain conditions on the payoff matrices, we devise a method that reduces the rank of the game without changing the equilibrium of the game. We leverage matrix pencil theory and the Wedderburn rank reduction formula to arrive at our results. We also present a constructive proof of the fact that in a generic square game, the rank of the game can be reduced by 1, and in generic rectangular game, the rank of the game can be reduced by 2 under certain assumptions.

==> 3dfigure.tex <==
\begin{tikzpicture}[xscale=0.8,>=latex]
% axis
% \draw (0,0) grid (13,4);
\draw[ultra thick,->] (0.3,-3.5) -- +(0,7) node[yshift=5pt] {};
\draw[ultra thick,->] (0.3,-3.5) -- +(220:4) node[yshift=-5pt,xshift=-5pt] {};
\draw[ultra thick,->] (0.3,-3.5) -- +(12,0) node[xshift=6pt] {};

% border of the surface1
\path[draw,name path=border1] (0,0) to[out=-10,in=150] (6,-2);
% border of the surface1
\path[draw,name path=border2] (12,1) to[out=150,in=-10] (5.5,3.7);
% border of the surface1
\draw[draw,thick,name path=line1] (6,-2) -- (12,1);
% border of the surface1
\path[draw,name path=line2] (5.5,3.7) -- (0,0);
% draw the surface1
\shade[left color=red!30,right color=red!10] 
  (0,0) to[out=-10,in=150] (6,-2) -- 
  (12,1) to[out=150,in=-10] (5.5,3.7) -- cycle;

% border of the surface2
\path[draw,name path=border3] (-1,-4) to[out=20,in=220] (3,3);
% border of the surface2
\path[draw,name path=border4] (6,-7) to[out=40,in=210] (9,1);
% border of the surface2
\path[draw,name path=border5] (-1,-4) to[out=0,in=80]  (6,-7);
% border of the surface2
\path[draw,name path=border6] (3,3) to[out=10,in=140] (9,1);
\node at (2,-5) {\Huge $A+B\in \mathcal C_k$};

% labels
% \node at (0.5,-3.8) {$\alpha$};
% \node at (10,1) {$\beta$};
% \node at (9.4,-4.5) (label) {$p_{\alpha\beta}(T)$};
% \draw[->] (label) -- +(185:3.35);

% draw the surface2
\shade[top color=gray!80,bottom color=gray!90,opacity=.30] 
  (-1,-4) to[out=20,in=220] (3,3)  to[out=10,in=140] (9,1)
 to[out=210,in=40] (6,-7) to[out=80,in=0] (-1,-4);

% intersection points
\path[name intersections={of=border3 and line2,by={a}}];
\path[name intersections={of=border4 and line1,by={b}}];

% intersection of the surfaces
\draw[thick,dashed] (a) to[out=-10,in=130] node[pos = 1.08,right,color = red] {\LARGE $\Big\{C = A+B:C_{12}^\transpose C_{11}^{-\transpose} \vct{1}_k = \vct{1}_{n-k}\Big\}$} (b);


% proyections of the intersection points
% \draw[help lines,gray!70] (a) -- +(0,-4.9) coordinate (proy1);
% \draw (b) -- +(0,-5) coordinate (proy2);

% proyection of the intersection path
% \draw[ultra thick] (proy1) to[out=0,in=130] (proy2);

\end{tikzpicture}

==> 3dfigureRank1.tex <==
\begin{tikzpicture}[xscale=0.8,>=latex]
% axis
% \draw (0,0) grid (13,4);
\draw[ultra thick,->] (0.3,-3.5) -- +(0,7) node[yshift=5pt] {};
\draw[ultra thick,->] (0.3,-3.5) -- +(220:4) node[yshift=-5pt,xshift=-5pt] {};
\draw[ultra thick,->] (0.3,-3.5) -- +(12,0) node[xshift=6pt] {};

% % border of the surface1
% \path[draw,name path=border1] (0,0) to[out=-10,in=150] (6,-2);
% % border of the surface1
% \path[draw,name path=border2] (12,1) to[out=150,in=-10] (5.5,3.7);
% % border of the surface1
% \draw[draw,thick,name path=line1] (6,-2) -- (12,1);
% % border of the surface1
% \path[draw,name path=line2] (5.5,3.7) -- (0,0);
% % draw the surface1
% \shade[left color=red!30,right color=red!10] 
%   (0,0) to[out=-10,in=150] (6,-2) -- 
%   (12,1) to[out=150,in=-10] (5.5,3.7) -- cycle;

% border of the surface2- left
\path[draw,name path=border3] (-1,-4) to[out=20,in=220] (3,3);
% border of the surface2 - right
\path[draw,name path=border4] (6,-7) to[out=20,in=210] (10,2);
% border of the surface2
\path[draw,name path=border5] (-1,-4) to[out=0,in=80]  (6,-7);
% border of the surface2 - top
\path[draw,name path=border6] (3,3) to[out=20,in=130] (10,2);
%\node at (2,-5) {\Huge $A+B\in \mathcal C_k$};
% path for a line crossing both borders
\path[name path=dashline] (2,-5) -- (7,4);

%intersections between the borders and the line
\path[name intersections={of=border5 and dashline,by={a}}];
\path[name intersections={of=border6 and dashline,by={b}}];

% draw the dashed line on the surface
\draw[dashed] (a) to[out=30,in=215] 
  coordinate[pos=0.2] (bux1) 
  coordinate[pos=0.5] (bux2) 
  coordinate[pos=0.8] (bux3) (b);
  
  %label the dashed line
  \node [yshift=-13pt] at (a) {\Large $\Re^{m+n+4}$};
  
  %label the surface
  \node [xshift=-5pt,yshift=-70pt] at (10,1) {\Large $\Re^{2m+2n+4}$};
  
  % Draw filled black circles on the line
  \draw[fill] (bux1) circle (3pt);
  \draw[fill] (bux3) circle (3pt);
  
  % Draw a filled black circle off the line
  \coordinate (offpath) at ([xshift=-37]bux2);
  \draw[fill] (offpath) circle (3pt);
  
  % Label the circles
  \node [xshift=49pt] at (bux1) {\large $(A,-A+\vec{r}\vec{c}^\transpose)$};
  \node [xshift=49pt] at (bux3) {\large $(\hat{A},-\hat{A}+\hat{\vec{r}}\hat{\vec{c}}^\transpose)$};
  \node [xshift=-23pt] at (offpath) {\large $(\tilde{A},\tilde{B})$};
  
  % Draw an arrow from (\tilde{A},\tilde{B}) to (\hat{A},-\hat{A})
%   \draw [-{Latex[length=3mm]}] (offpath) -- ([xshift=-2,yshift=-2]bux3);

% border of the surface2- left
%\path[draw,name path=border3] (-1,-4) to[out=20,in=220] (3,3);
% border of the surface2 - right
%\path[draw,name path=border4] (6,-7) to[out=20,in=210] (10,2);
% border of the surface2
%\path[draw,name path=border5] (-1,-4) to[out=0,in=80]  (6,-7);
% border of the surface2 - top
%\path[draw,name path=border6] (3,3) to[out=20,in=130] (10,2);

% draw the surface2
\shade[top color=gray!80,bottom color=gray!90,opacity=.30] 
  (-1,-4) to[out=20,in=220] (3,3)  to[out=20,in=130] (10,2)
 to[out=210,in=20] (6,-7) to[out=80,in=0] (-1,-4);

% intersection points
% \path[name intersections={of=border3 and line2,by={a}}];
% \path[name intersections={of=border4 and line1,by={b}}];

% % intersection of the surfaces
% \draw[thick,dashed] (a) to[out=-10,in=130] node[pos = 1.08,right,color = red] {\LARGE $\Big\{C = A+B:C_{12}^\transpose C_{11}^{-\transpose} \vct{1}_k = \vct{1}_{n-k}\Big\}$} (b);


% proyections of the intersection points
% \draw[help lines,gray!70] (a) -- +(0,-4.9) coordinate (proy1);
% \draw (b) -- +(0,-5) coordinate (proy2);

% proyection of the intersection path
% \draw[ultra thick] (proy1) to[out=0,in=130] (proy2);

\end{tikzpicture}
